Neuroflight: Next Generation Flight Control Firmware

Little innovation has been made to low-level attitude flight control used by uncrewed aerial vehicles (UAVs), which still predominantly uses the classical PID controller. In this work we introduce Neuroflight, the first open source neuro-flight controller firmware. We present our toolchain for training a neural network in simulation and compiling it to run on embedded hardware. Challenges faced jumping from simulation to reality are discussed along with our solutions. Our evaluation shows the neural network can execute at over 2.67kHz on an Arm Cortex-M7 processor and flight tests demonstrate a quadcopter running Neuroflight can achieve stable flight and execute aerobatic maneuvers.

==> bg.tex <==
\subsection{Reinforcement learning}
\subsection{Flight Control System Architecture}

PID Mix vs NN based control 

Basic dynamics
how to achieve tranlational movement? rotate then thrust

different levels of control, inner loop and outter loop

\missingfigure{Overview of the architecture of a flight control system I/O}

The control signal output ($y_i$) represents a percentage of the power to be
delivered to motor $i$ in the range $[0,1]$ where 0.0 is no rotation of the
motor and 1.0
is max rotation. 


==> discuss.tex <==
Pros

Cons

* Loop speed - What is the max sampling? This is some kinda of law
PID has far less arithmetic operations



What is the minimum model we need to generate a FC?

